VIS30K: A Collection of Figures and Tables from IEEE Visualization Conference Publications

We present the VIS30K dataset, a collection of 29,689 images that represents 30 years of figures and tables from each track of the IEEE Visualization conference series (Vis, SciVis, InfoVis, VAST). VIS30K's comprehensive coverage of the scientific literature in visualization not only reflects the progress of the field but also enables researchers to study the evolution of the state-of-the-art and to find relevant work based on graphical content. We describe the dataset and our semi-automatic collection process, which couples convolutional neural networks (CNN) with curation. Extracting figures and tables semi-automatically allows us to verify that no images are overlooked or extracted erroneously. To improve quality further, we engaged in a peer-search process for high-quality figures from early IEEE Visualization papers. With the resulting data, we also contribute VISImageNavigator (VIN, visimagenavigator.github.io), a web-based tool that facilitates searching and exploring VIS30K by author names, paper keywords, title and abstract, and years.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Sections/7.Conclusion.tex <==

%\section{Conclusion}
%\label{sec:conclusion}
%
%We introduce a meticulously curated figure and table dataset of IEEE VIS conference publications over its entire 30-year history. The dataset is used to provide three data-exploration tools and a gateway for exploration on Google Drive for scholars to answer scientific questions.



%Our \%2 approach can produce any scholarly article corpus of any format.  \$2 is image-based and thus does not require any schema-based content (e.g., XML). As a result, our approach has a more generalized ability to extract data from any document collection, such as the earlier years when XML contents are not readily available.




==> Sections/Extraction2long.tex <==

%We now describe the concrete steps in our algorithm to prepare labelled ground-truth training data by synthetic paper composition. 
The essential part of our approach is to treat training data as a composition of individual document elements, where the goals are (1) to record bounding boxes for each of the labels/component parts in a PDF image to produce high-quality labels for the training data; and (2) to synthesize appearance to minimize the differences between the training data and the real paper to some extent. 

Our method is based on the observation that scholarly visualization documents are typically highly structured and formatted following certain format guidelines. 
To find the document entities and their composition, 
we began with collecting VIS paper PDFs. We browsed the dataset to understand what entities were present and what properties might influence CNN figure-extraction accuracy.
We had the following observations.

\begin{itemize}

\item 
\textbf{Observation \#1.}
Since these are structured scientific publications, we assume a consistent structural appearance: (i) a first page with title and abstract, (ii) an inner page with or without figures, (iii) figures spanning a single column or two columns, and (iv) a last page that contains an arbitrary number of lines. 

\item
\textbf{Observation \#2.}
Although the specific paper format has changed over the years, the papers generally have a consistently structured layout: (1) main text, (2) headers (journal name and authors), (3) single- or double-column abstracts, (4) figures, (5) tables, (6) figure and table captions, (7) bullet lists, and (8) equations. 

\item
\textbf{Observation \#3. }
Figures and tables can occupy a single or double column size to fit one column or page width at a scale defined by authors. These scales are often between [0.5, 1]. There are also inline figures and figures that do not have captions. 
The white space between figures can range from large or small to none. We also noticed certain image characteristics. In particular, often papers from the earlier years are in black-and-white, including some unidentifiable images due to low scan quality.

\item
\textbf{Observation \#4.}
Abstracts in the earlier years are in single column format, changing to double-column format when papers became published in the \textit{IEEE Transactions on Visualization and Computer Graphics}.

\end{itemize}

\begin{comment}
We used these observations to customize particular formats of paper pages. Teasing apart these paper page elements allows our approach to be easily customized to any specific page patterns, as opposed to having to extract the component parts of a paper page or rules by hand. 
\todo[inline]{this is a bold claim, not supported by anything you have done.}
\end{comment}




\subsubsection{Textual Content}
Following the first two observations above, we assembled the textual content (\textit{body text}  depicted in particular coordinates with particular fonts and styles, \textit{document headers}, \textit{paper titles}, \textit{paper abstracts}, \textit{captions}, \textit{bullets and equations}) using Stribling et al.'s \cite{stribling2005scigen} SCIgen algorithm.
%, so that the paragraphs when used were coherent. 
We generated paragraphs and inserted them into our rendering to match the structure. The actual text did not matter as we were only interested in identifying the paper figures. We also inserted \textit{bullets and equations} because our pilot studies revealed that without this class label, bullets and equations from the real-paper were often mis-classified as \textit{points}, a figure type.
%\ms{again, this seems to be a left over from the analysis classification idea ... so far, the only goal we outline is image and table extraction}
We specified the abstract to be 6--15 lines long, the title to be at most 20 words, and captions to be no more than 6 lines long; this setting covers the majority of the content format. 


\subsubsection{Figure and Table Corpus}

To reduce the requisite number of images and promote design variability, we re-purposed images from the MASSVIS dataset (http://massvis.mit.edu/) collected by Borkin et al.~\cite{borkin2013makes}. 
We chose this set due to its broad coverage of science and web visualization images. We removed those figures with abundant textual content that would rarely appear in visualization papers to improve the similarity of the remaining infographics images to the IEEE VIS figures. We removed an image if it contained what is called chart junks and only kept those closely resembling paper images we had observed. This left us 74 area and pie charts, 181 bar charts, 165 line charts, 134 maps, 31 matrices, 60 photos, 65 point chart, 116 tables, 67 trees and network visualizations, and 230 figures containing more than one chart type. 
%The MASSVIS dataset also contained about 60 items from the photo category which we retained as visualization papers also sometimes contain photographs. 
%\textcolor{red}{I don't understand this next sentence and why it is here:} We added some of the visualization scholars' photos at different stages of their career with the intent to honor them and and photos of political leaders (\eg, the Biden family).
%Though excluded in our VIS29K collection, in the long run we would like to have a model capable of extracting keynote speakers' and authors' photos from the TVCG collections presented at VIS.
%This dataset is also labeled as area chart, line chart, bar chart, etc.
Since the MASSVIS dataset focused on infographics, we also randomly sampled 131 spatial data visualization techniques from Li and Chen's~\cite{li2018toward} analysis of the memorability of SciVis paper images to diversify the training data to extract images from papers in the entire visualization conference. 
This process resulted in 1,254 figure and table samples in total.

Papers from earlier years were black and white and might have the salt-and-pepper type of image noisy. This variation in image appearance such as brightness or contrast can work against our CNN's image detection accuracy. To match these visual characteristics, we doubled the 1,254 figure/table samples to 2,508 images by changing these images to black and white images, with various gray-scale variations. 
In total we produced 2,508 input images with 10 figure class labels (area and pie, bar, line, maps, matrix, photos, points, sciVis, tree and networks, multiples), and a table class listed in ~\autoref{fig:workflow}.
\todo[inline]{this should say 'Figure' but says 'section'}
%\textcolor{red}{[How many? I count 1263 in total from the above, so is it correct that you added 101 images to get to the total of 1364?] [And how selected, randomly?]} 
%\textcolor{blue}{[1254 from the original figure+table classes; 2508 from the whole set after gray-scale transform. Please see next note why double.]}


\subsubsection{Annotated Paper Page Synthesis}

We used the text and our limited figure and table corpus to automatically synthesize a large set of papers. We first created a blank image with a default $1075\times1400$ pixel resolution. Depending on the page format (Observation \#1),
we inserted the header, and the title and abstract first. The Month entry and the \textit{vol.} numbers in the headers were randomly created. 
We then chose a random number of images ($\leq{2}$) from the figure and table cohort, rescale the image with a random scaling factor to fit the image width to 50-200\% column width (Observation \#3), and finally insert this image at a random vertical pixel location. The image is always centered in one or two columns.
%We applied a random scaling \textcolor{red}{ between 0.5 and 1 to insert \textcolor{red}{[what]} to text pages.
We next added captions underneath figures and tables.
Finally, we inserted body text in the white space and randomly broke the sentences into paragraphs. 
We recorded the accurate bounding box locations and sizes in this process. 
%\textcolor{red}{[Why? There are examples without captions in the corpus.]}  
%\textcolor{blue}{[Why? See below. I admitted this and indeed most small figures were not detected. I believe this has something to do with my image scale-configuration (50\%-200\% column width. I could have used say 20\% column width. I will improve this configuration in the next classifier.}  


As a proof-of-concept of our learning algorithm, we left out %harder 
cases such as iconic figures without captions and inline figures. We also only used the current VIS paper format to position the title, abstract, main text, bullets and equations, and captions, and did not create subsections. Even with this proof-of-concept technique for configuring synthesized paper training examples, we found that CNNs provided reasonable accuracy of the trained classier for both the earlier and recent years.
Our classifier, however, failed to extract some of the very small figures. 
%Given that we have a very limited knowledge of CNN's behavior for document training set production,  our work  provides the community an opportunity to examine how page configuration complexity would influence prediction outcome of the classifiers. \todo[inline]{drop that last sentence, it is not needed, opens a can of worms and is hard to understand.}
%\ms{can we give accuracy numbers?} 
%\textcolor{red}{[Why not also the old template? Was it no longer available?]}
%\textcolor{blue}{[Thanks for the note. I added a paragraph to admit this. This parameter is perhaps not important from the already-structured papers. 
%It is easy to implement. Format-wise, I simply used a ruler to measure the page configuration. 
%One reason was that I ran out of time after non-stop programming for two days, so I ranked the parameters and determined this was not on top of my list.
%My current training data production is to minimize the complexity in the production process to reduce the \# of training samples and save training time.Maybe a CHI paper idea: we let users interactively compose and draw their own paper format, use my algorithm to create training samples, train the classifier, and then return the models or the results to the users in two days.]}
%Also, because we know the locations where images are inserted, 
%This simple solution avoids the time-consuming and laborious effort of manually labeling actual papers and provides an alternative to data generation for training neural networks. 
%\textcolor{red}{[Did you mix the grayscale images with everything or did you just randomly select images from the pool? After all, the old papers will only have grayscale images, and the new ones will have mostly colored images.]}
%\textcolor{blue}{[you are correct. The number of images doubled. This is because CNN does not like the long-tail distributions. If a class falls into the long-tail, CNN would almost never find it (CNN might have treated the data as noise.) So even if we have only a few black blogs images, we still need to produce many samples in order to find them.]}

In total, we generated 13,000 pages (10,000 for training and 3,000 for validation), each having dimensions of 1075\,\texttimes\,1400 pixels and labeled by up to 17 class tags (1. body text; 2. title; 3. abstract; 4. header; 5. caption; 6. Bullets and equations; 
7. area and circular chart; 8. bar chart; 9. line chart; 10. map; 11. matrix view and parallel coordinates; 12. multi-types (visualization that contains multiple types of visualizations);
%\todo[inline]{do you mean 'multiple types of vis'?}; 
13. photos; 14. point cloud; 15. SciVis; 16. Tables; and 16. Tree and network.) All these tags have accurate bounding box locations.


==> Sections/Extraction3long.tex <==

Next we trained
two complementary CNN approaches, YOLOv3~\cite{redmon2018yolov3,redmon2016you} and  Faster R-CNN~\cite{ren2015faster}, independently for subsequent figure extraction from the actual papers. One may think about this combination as a means to boost performance of our learning algorithm since we only use a small set of labelled examples.

YOLOv3 is a single-stage detector network, and is fast and accurate for object detection. 
%outputs are generated from every single cell in the feature space.
The second Faster R-CNN~\cite{ren2015faster} is a multi-stage proposal and sampling-based approach, where a certain number of candidates were sampled from a large pool of generated ROIs. 
%prediction results were produced by repeatedly cropping the corresponding regions on feature maps.
%the number of predictions is proportional to the number of samples.
Both YOLOv3 and Faster-RCNN returned the four coordinates of each bounding box, along with a class label. 
%The rationale for choosing these two CNN methods is that we found during initial experimentation that Faster R-CNN is a better localization method that provides more precise bounding boxes, while YOLOv3 provides a better detection with less misses.

We implemented the training of both models under TensorFlow with a single GPU. For YOLOv3 we used the following properties: we used DarkNet-53 as the backbone, an initial learning rate of $10^{-4}$ that decays to $10^{-6}$, in 60 to 80 epochs with a batch size of 6. For Faster-RCNN, we used ResNet-101 (101 layers deep) as the backbone and turned on FPN (feature pyramid network) and Cascade R-CNN. We used the base learning rate of $10^{-2}$, which was adjusted automatically during the training. The model is typically trained in a similar number of epochs as used by YOLOv3, but with a batch size of 1 and requires a much longer time. Both models take an input image of arbitrary resolution and resize/pad it to a certain input size, before feeding it into the model. The input size ranges from 320--608 pixels for YOLOv3 and 640--800 pixels for Faster-RCNN. We monitored the mean average precision (mAP) and the bounding box precision on the validation set to make model adjustment and to compare the relative performance of the two models.
%Training and validation of Faster-RCNN and YOLOv3 are the same. 

In the prediction stage, we used the paper PDFs that we downloaded by following the links in the VisPubData database~\cite{isenberg2016vispubdata}. Excluding short papers, posters, panels, and keynote files, this resulted in a collection of 2,916 full papers for the years 1990--2019. We then first converted these PDFs to JPEG images using the UNIX command \textit{convert} with a density of 200 DPI, yielding images that ranged from 1500 to 1600 pixels in width and 2050 to 2200 pixels in height. 
We then fed these JPEGs into the CNNs to obtain the labels of figures, tables, captions, etc.

After processing, we combined the two models' labeling results by merging the bounding boxes captured by Faster R-CNN (better localization) with any additional images detected and labeled by YOLOv3 (better detection) to create the initial set of predictions. 
We further tightened or expanded labeled bounding boxes to acquire accurate regions for each figure and table.

